Timed Strategies for Real-Time Rewrite Theories

In this paper we propose a language for conveniently defining a wide range of execution strategies for real-time rewrite theories, and provide Maude-strategy-implemented versions of most Real-Time Maude analysis methods, albeit with user-defined discrete and timed strategies. We also identify a new time sampling strategy that should provide both efficient and exhaustive analysis for many distributed real-time systems. We exemplify the use of our language and its analyses on a simple round trip time protocol, and compare the performance of standard Maude search with our strategy-implemented reachability analyses on the CASH scheduling algorithm benchmark.

==> rtm-analysis.tex <==
\section{Performing Real-Time Maude Analyses using Maude's Strategy Language}
\label{sec:rtm-analysis}

In this section we show how the different analysis methods  supported
by Real-Time Maude can be performed using Maude and executions using
its strategy language. The key issue is to use strategies to
``implement'' Real-Time Maude time sampling and time-bounded analyses.

\textbf{Should these be defined directly in Maude's strategy language,
  or using the NEW language Carlos is defining??}

\textbf{Do we have results on this?}



==> strat-lang.tex <==
\section{A User-Friendly Strategy Language for Timed Rewrite Strategies}
\label{sec:strat-lang}

\textbf{``User-friendly''?  ``Intuitive''?  ``Simple''?  Is it a
  general strategy language, or   mostly for timed systems??  The
  header shoud be polished.}

\textbf{This is Carlos language, right?}


